GeV Observations of Star-forming Galaxies with \textit{Fermi} LAT

Recent detections of the starburst galaxies M82 and NGC 253 by gamma-ray telescopes suggest that galaxies rapidly forming massive stars are more luminous at gamma-ray energies compared to their quiescent relatives. Building upon those results, we examine a sample of 69 dwarf, spiral, and luminous and ultraluminous infrared galaxies at photon energies 0.1-100 GeV using 3 years of data collected by the Large Area Telescope (LAT) on the \textit{Fermi Gamma-ray Space Telescope} (\textit{Fermi}). Measured fluxes from significantly detected sources and flux upper limits for the remaining galaxies are used to explore the physics of cosmic rays in galaxies. We find further evidence for quasi-linear scaling relations between gamma-ray luminosity and both radio continuum luminosity and total infrared luminosity which apply both to quiescent galaxies of the Local Group and low-redshift starburst galaxies (conservative $P$-values $\lesssim0.05$ accounting for statistical and systematic uncertainties). The normalizations of these scaling relations correspond to luminosity ratios of $\log(L_{0.1-100 \rm{GeV}}/L_{1.4 \rm{GHz}}) = 1.7 \pm 0.1_{\rm (statistical)} \pm 0.2_{\rm (dispersion)}$ and $\log(L_{0.1-100 \rm{GeV}}/L_{8-1000 \mu\rm{m}}) = -4.3 \pm 0.1_{\rm (statistical)} \pm 0.2_{\rm (dispersion)}$ for a galaxy with a star formation rate of 1 $M_{\odot}$ yr$^{-1}$, assuming a Chabrier initial mass function. Using the relationship between infrared luminosity and gamma-ray luminosity, the collective intensity of unresolved star-forming galaxies at redshifts $0<z<2.5$ above 0.1 GeV is estimated to be 0.4-2.4 $\times 10^{-6}$ ph cm$^{-2}$ s$^{-1}$ sr$^{-1}$ (4-23% of the intensity of the isotropic diffuse component measured with the LAT). We anticipate that $\sim10$ galaxies could be detected by their cosmic-ray induced gamma-ray emission during a 10-year \textit{Fermi} mission.

==> app_sec_seyfert.tex <==
\section{Origin of the High-Energy Emission from Seyfert 2 Galaxies}\label{sec:Seyfert}

A large fraction of Seyfert galaxies also contain circumnuclear
starbursts and it has been proposed that the two phenomena may be connected in the evolution of
galaxies (reviewed by Heckman 2008). The Seyfert II galaxies NGC 1068 and NGC 4945 are two of
the most extensively studied examples of this composite starburst-AGN behavior. 

\subsection{NGC 1068}

The first clear indications for an AGN within NGC 1068 came with the
discovery of polarized optical continuum emission (Miller \& Antonnuci
1983) and broad line emission (Antonnuci \& Miller 1985) towards the
nuclear region. 
Shortly afterward, Wilson \& Ulvestad (1987)
identified two opposing kpc-scale jets at radio frequencies
which produce bow shocks in the ISM. Milliarcsecond
VLBA imaging at 1.4 and 5 GHz resolved discrete knots along the radio
jet and identified a nuclear radio counterpart of 0.8 pc in scale distinguished by an inverted radio spectrum 
(Gallimore 2004). The compact nuclear source is likely associated with
a geometrically thin maser disk, but in spite of additional multiwavelength
data, interpretation of the radio emission from this
innermost region as either synchrotron or thermal free-free emission
is uncertain (H\"{o}nig et al. 2008). The jet is relatively weak,
constrained to a velocity $\lesssim5\times10^{4}$ km s$^{-1}$
(Gallimore at el. 1996) and has likely been deflected by the
interaction with a molecular cloud (M\"{u}ller-S\'{a}nchez et al. 2009). The
radio-quiet nature of NGC 1068 is substantially different from the misaligned radio-loud AGN previously
detected by the LAT (Abdo et al. 2010f).

Lenain et al. (2010) argued that the GeV emission from NGC 1068 is
primarily related to the AGN rather than diffuse CR interactions
associated with the starburst. Part of this argument was based
on the observation that the gamma-ray luminosity of NGC 1068 is
substantially higher than that of the other LAT-detected starbursts,
while the estimated supernova rate (0.20$\pm$0.08 yr$^{-1}$, using the
$L_{{\rm FIR}}$-supernova rate relation proposed by Mannucci et al. 2003)
was only comparable to the other galaxies. In other words, some doubt
existed as to whether a starburst with the quoted supernova rate could
fully explain the measured gamma-ray luminosity. However, comparisons
between supernova rates are difficult to interpret unless consistent
estimators are used for each object in a sample since different
systematics affect each estimator. An examination of Table \ref{candidates}
shows that RC luminosity, total IR luminosity, and HCN luminosity of
NGC 1068, each an independent tracer of massive star-formation, are
all approximately an order of magnitude larger in comparison to M82, NGC 253,
and NGC 4945. However, these photometric estimators of SFR may suffer
influences from the AGN. Approximately 80\% of the RC emission at 1.4
GHz comes from the region coinciding with the central outflow (Wilson
\& Ulvestad 1982), and nuclear emission is dominant in the mid-IR
shortward of $\sim30$ $\mu$m (Spinoglio 2005). NGC 1068
also appears to have anamolous molecular gas chemistry, notably in that the HCN/CO ratio is
unusually large relative to other LIRGs, which may be an effect of
strong X-ray emission (Usero et al. 2004; Juneau
2009). Nevertheless, evidence for intense star-formation in a
circumnuclear ring $\sim3$ kpc in radius is found in spatially
extended RC and IR emission, as well as near-IR emission
lines (Davies et al. 1998), and the UV continuum (Neff et al. 1994),
all of which coincide with knots of molecular gas traced by CO emission. \textit{Chandra} observations of
compact X-ray sources show that the number of X-ray binary candidates in NGC
1068 is approximately 4 times larger than the number found in M82, a futher indicator of
recent formation of massive stars, though with limited statistics (Smith \&
Wilson 2003). In the nuclear region, episodic starburst activity appears to
be fueled by the inflow of molecular gas towards the accretion disk
(Davies et al. 2007).

\subsection{NGC 4945}

The nuclear region of NGC 4945 exhibits both starburst and AGN
characteristics including a high IR flux exceeded only by M82 and
NGC 253, H$_{2}$O maser emission, a discrete radio source with flatter spectrum compared to the
surrounding diffuse emission (Whiteoak 1986), and is one of the
brightest extragalactic hard X-ray sources in the sky (Done et al. 1996). This galaxy lacks the larger-scale
radio jet features of NGC 1068, but does contain a possible pc-scale
structure with jet-like morphology offset from the expected AGN
location by $\sim20$ pc (Lenc \& Tingay 2009). The distances, RC
luminosities and IR luminosities, dense gas
quantities, and supernova rates (Lenc \& Tingay 2009) of M82, NGC 253, and NGC 4945 are all comparable.

==> table_ir_detail.tex <==
\begin{table}\tiny %\scriptsize, \tiny
\begin{center}
\caption{Galaxy luminosities at specific IR wavelengths}
\label{table_ir_detail}
\begin{tabular}{c cccc}
\\
\toprule
Galaxy & $L_{12 \mu\rm{m}}$ & $L_{25 \mu\rm{m}}$ & $L_{60 \mu\rm{m}}$ & $L_{100 \mu\rm{m}}$ \\
 & (10$^{23}$ W Hz$^{-1}$) & (10$^{23}$ W Hz$^{-1}$) & (10$^{23}$ W Hz$^{-1}$) & (10$^{23}$ W Hz$^{-1}$) \\
\midrule
LMC & 0.00832 & 0.0234 & 0.248 & 0.253 \\
SMC & 0.000289 & 0.00116 & 0.0288 & 0.0647 \\
M31 & 0.122 & 0.0804 & 0.400 & 2.19 \\
M33 & 0.0276 & 0.0340 & 0.354 & 1.06 \\
MW & 1.22 & 0.722 & 1.62 & 4.62 \\
NGC 253 & 0.307 & 1.16 & 7.24 & 9.63 \\
M82 & 1.10 & 4.60 & 20.5 & 19.0 \\
IC 342 & 0.244 & 0.565 & 2.96 & 6.42 \\
NGC 4945 & 0.454 & 0.694 & 10.2 & 21.8 \\
M83 & 0.352 & 0.714 & 4.35 & 8.58 \\
NGC 4826 & 0.0624 & 0.0756 & 0.970 & 2.16 \\
NGC 6946 & 0.438 & 0.749 & 4.70 & 10.5 \\
NGC 2903 & 0.243 & 0.397 & 2.78 & 6.00 \\
NGC 5055 & 0.341 & 0.406 & 2.55 & 8.92 \\
NGC 3628 & 0.216 & 0.335 & 3.79 & 7.31 \\
NGC 3627 & 0.333 & 0.591 & 4.58 & 9.44 \\
NGC 4631 & 0.405 & 0.704 & 6.70 & 12.6 \\
NGC 4414 & 0.288 & 0.374 & 3.06 & 7.32 \\
M51 & 0.795 & 1.05 & 10.7 & 24.4 \\
NGC 891 & 0.669 & 0.889 & 8.44 & 21.9 \\
NGC 3556 & 0.308 & 0.563 & 4.38 & 10.3 \\
NGC 3893 & 0.335 & 0.381 & 3.60 & 8.51 \\
NGC 660 & 0.715 & 1.71 & 15.4 & 26.9 \\
NGC 5005 & 0.387 & 0.530 & 5.20 & 14.9 \\
NGC 1055 & 0.587 & 0.744 & 6.12 & 17.1 \\
NGC 7331 & 1.06 & 1.59 & 12.1 & 29.7 \\
NGC 2146 & 1.89 & 5.20 & 40.6 & 53.6 \\
NGC 3079 & 0.798 & 1.13 & 15.9 & 32.9 \\
NGC 1068 & 13.3 & 29.2 & 65.5 & 85.9 \\
NGC 4030 & 0.472 & 0.805 & 6.47 & 17.8 \\
NGC 4041 & 0.438 & 0.605 & 5.49 & 12.3 \\
NGC 1365 & 2.65 & 7.39 & 48.8 & 85.8 \\
NGC 1022 & 0.378 & 1.75 & 10.5 & 14.6 \\
NGC 5775 & 0.993 & 1.34 & 12.8 & 30.2 \\
NGC 5713 & 1.01 & 1.96 & 15.2 & 25.7 \\
NGC 5678 & 0.869 & 1.11 & 8.94 & 23.7 \\
NGC 520 & 1.04 & 3.73 & 36.5 & 54.8 \\
NGC 7479 & 2.03 & 5.72 & 22.1 & 39.6 \\
NGC 1530 & 1.08 & 1.84 & 14.8 & 38.7 \\
NGC 2276 & 1.61 & 2.46 & 21.5 & 43.7 \\
NGC 3147 & 3.64 & 1.92 & 15.3 & 55.3 \\
Arp 299 & 8.78 & 54.2 & 250 & 246 \\
IC 5179 & 3.01 & 6.13 & 49.5 & 95.2 \\
NGC 5135 & 2.01 & 7.61 & 53.9 & 99.0 \\
NGC 6701 & 2.12 & 5.10 & 38.8 & 77.4 \\
NGC 7771 & 4.32 & 9.47 & 85.9 & 175 \\
NGC 1614 & 6.60 & 35.8 & 154 & 164 \\
NGC 7130 & 2.93 & 10.9 & 84.5 & 131 \\
NGC 7469 & 8.67 & 32.5 & 149 & 192 \\
IRAS 18293-3413 & 7.09 & 24.8 & 222 & 332 \\
Arp 220 & 4.07 & 53.4 & 695 & 770 \\
Mrk 331 & 3.53 & 17.2 & 122 & 154 \\
NGC 828 & 4.90 & 7.28 & 78.0 & 172 \\
IC 1623 & 8.23 & 29.2 & 183 & 252 \\
Arp 193 & 2.57 & 14.6 & 175 & 251 \\
NGC 6240 & 6.79 & 40.9 & 264 & 305 \\
NGC 1144 & 4.58 & 10.4 & 87.3 & 187 \\
Mrk 1027 & 4.74 & 11.3 & 96.4 & 156 \\
NGC 695 & 10.7 & 17.7 & 162 & 289 \\
Arp 148 & 4.91 & 17.4 & 157 & 253 \\
Mrk 273 & 6.65 & 65.4 & 624 & 624 \\
UGC 05101 & 7.68 & 31.3 & 359 & 611 \\
Arp 55 & 4.43 & 19.3 & 192 & 327 \\
Mrk 231 & 63.5 & 307 & 1070 & 1030 \\
IRAS 05189-2524 & 25.7 & 120 & 460 & 411 \\
IRAS 17208-0014 & 7.17 & 57.7 & 1150 & 1290 \\
IRAS 10566+2448 & 7.19 & 45.6 & 435 & 539 \\
VII Zw 31 & 11.9 & 37.0 & 329 & 603 \\
IRAS 23365+3604 & 7.63 & 79.6 & 630 & 763 \\
\bottomrule
\end{tabular}
\end{center}
\tablenotetext{}{Except for the Milky Way, luminosities are taken from
  \cite{sanders_2003_iras_rbgs} and re-scaled to the distances listed in
  Tables \ref{table_candidates} and \ref{table_local_group} for
  consistency. The global Milky Way IR spectrum is that used by \cite{strong_2010_global} to model
  the interstellar radiation field.}
\end{table}

==> table_regression_no_agn.tex <==
\begin{table}\footnotesize
\begin{center}
\caption{Scaling relationships between global luminosities: power-law
  fits excluding galaxies hosting \textit{Swift}-BAT AGN}
\label{regression}
\begin{tabular}{c ccc ccc}
\\
\toprule
 & \multicolumn{3}{c}{Expectation-Maximization Method} & \multicolumn{3}{c}{Buckley-James Method} \\
 & $\alpha$ & $\beta$ & $\sqrt{{\rm Variance}}$ & $\alpha$ & $\beta$ & $\sqrt{{\rm Variance}}$ \\
\midrule
$L_{1.4 \; {\rm GHz}}$ : $L_{0.1--100 {\rm GeV}}$ & 1.10 $\pm$ 0.07 & 38.81 $\pm$ 0.07 & 0.19 & 1.09 $\pm$ 0.11 & 38.80 & 0.24 \\
(10$^{21}$ W Hz$^{-1}$) : (erg s$^{-1}$) & & & & & & \\
\midrule
$L_{8-1000 \; \mu {\rm m}}$ : $L_{0.1--100 {\rm GeV}}$ & 1.09 $\pm$ 0.10 & 39.19 $\pm$ 0.10 & 0.25 & 1.10 $\pm$ 0.14 & 39.22 & 0.33 \\
(10$^{10}$ $L_{\odot}$) : (erg s$^{-1}$) & & & & & & \\
\midrule
$L_{12 \mu {\rm m}}$ : $L_{0.1--100 {\rm GeV}}$ & 0.75 $\pm$ 0.14 & 39.47 $\pm$ 0.22 & 0.44 & 0.75 $\pm$ 0.19 & 39.48 & 0.60 \\
(10$^{23}$ W Hz$^{-1}$) : (erg s$^{-1}$) & & & & & & \\
\midrule
$L_{25 \mu {\rm m}}$ : $L_{0.1--100 {\rm GeV}}$ & 0.88 $\pm$ 0.09 & 39.43 $\pm$ 0.12 & 0.26 & 0.88 $\pm$ 0.12 & 39.45 & 0.34 \\
(10$^{23}$ W Hz$^{-1}$) : (erg s$^{-1}$) & & & & & & \\
\midrule
$L_{60 \mu {\rm m}}$ : $L_{0.1--100 {\rm GeV}}$ & 1.11 $\pm$ 0.08 & 38.71 $\pm$ 0.08 & 0.21 & 1.11 $\pm$ 0.12 & 38.71 & 0.28 \\
(10$^{23}$ W Hz$^{-1}$) : (erg s$^{-1}$) & & & & & & \\
\midrule
$L_{100 \mu {\rm m}}$ : $L_{0.1--100 {\rm GeV}}$ & 1.21 $\pm$ 0.08 & 38.36 $\pm$ 0.07 & 0.18 & 1.20 $\pm$ 0.11 & 38.36 & 0.23 \\
(10$^{23}$ W Hz$^{-1}$) : (erg s$^{-1}$) & & & & & & \\
\bottomrule
\end{tabular}
\end{center}
\tablenotetext{}{As Table \ref{table_regression}, but considering the subsample galaxies not hosting AGN detected by the
\textit{Swift}-BAT (60 objects).}
\end{table}
